ASNets: Deep Learning for Generalised Planning

In this paper, we discuss the learning of generalised policies for probabilistic and classical planning problems using Action Schema Networks (ASNets). The ASNet is a neural network architecture that exploits the relational structure of (P)PDDL planning problems to learn a common set of weights that can be applied to any problem in a domain. By mimicking the actions chosen by a traditional, non-learning planner on a handful of small problems in a domain, ASNets are able to learn a generalised reactive policy that can quickly solve much larger instances from the domain. This work extends the ASNet architecture to make it more expressive, while still remaining invariant to a range of symmetries that exist in PPDDL problems. We also present a thorough experimental evaluation of ASNets, including a comparison with heuristic search planners on seven probabilistic and deterministic domains, an extended evaluation on over 18,000 Blocksworld instances, and an ablation study. Finally, we show that sparsity-inducing regularisation can produce ASNets that are compact enough for humans to understand, yielding insights into how the structure of ASNets allows them to generalise across a domain.

==> code-samples/style.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother


\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> results/det-figures/blocks.tex <==
% ASNets & ASNets (PE) & ASNets (no h.) & A* (adm.) & A* (inadm.) & GBF (adm.) & LAMA-2011 & LAMA-first \\
blocks-nblk35-seed2107726020-seq1 &\wskip
  & 110 % ASNets
  & 119 (10/10) % ASNets (PE)
  & 108 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 138 % LAMA-2011
  & 138 % LAMA-first
  \\
blocks-nblk35-seed2107726020-seq10 &\wskip
  & 106 % ASNets
  & 113.6 (10/10) % ASNets (PE)
  & 104 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 116 % LAMA-2011
  & 116 % LAMA-first
  \\
blocks-nblk35-seed2107726020-seq2 &\wskip
  & 108 % ASNets
  & 120.2 (10/10) % ASNets (PE)
  & 112 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 108 % LAMA-2011
  & 162 % LAMA-first
  \\
blocks-nblk35-seed2107726020-seq3 &\wskip
  & 98 % ASNets
  & 111.6 (10/10) % ASNets (PE)
  & 100 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 108 % LAMA-2011
  & 170 % LAMA-first
  \\
blocks-nblk35-seed2107726020-seq4 &\wskip
  & 110 % ASNets
  & 125.2 (10/10) % ASNets (PE)
  & 120 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 134 % LAMA-2011
  & 228 % LAMA-first
  \\
blocks-nblk35-seed2107726020-seq5 &\wskip
  & 114 % ASNets
  & 133.6 (10/10) % ASNets (PE)
  & 108 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 146 % LAMA-2011
  & 166 % LAMA-first
  \\
blocks-nblk35-seed2107726020-seq6 &\wskip
  & 102 % ASNets
  & 111 (10/10) % ASNets (PE)
  & 102 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 110 % LAMA-2011
  & 110 % LAMA-first
  \\
blocks-nblk35-seed2107726020-seq7 &\wskip
  & 96 % ASNets
  & 97 (10/10) % ASNets (PE)
  & 96 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 262 &\wskip % GBF (adm.)
  & 102 % LAMA-2011
  & 118 % LAMA-first
  \\
blocks-nblk35-seed2107726020-seq8 &\wskip
  & 108 % ASNets
  & 114.8 (10/10) % ASNets (PE)
  & 106 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 290 &\wskip % GBF (adm.)
  & 114 % LAMA-2011
  & 160 % LAMA-first
  \\
blocks-nblk35-seed2107726020-seq9 &\wskip
  & 106 % ASNets
  & 125.8 (10/10) % ASNets (PE)
  & 114 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 114 % LAMA-2011
  & 116 % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq1 &\wskip
  & 158 % ASNets
  & 181 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq10 &\wskip
  & 146 % ASNets
  & 162.4 (10/10) % ASNets (PE)
  & 154 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq11 &\wskip
  & 158 % ASNets
  & 197.4 (10/10) % ASNets (PE)
  & 172 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq12 &\wskip
  & 150 % ASNets
  & 161 (10/10) % ASNets (PE)
  & 146 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 200 % LAMA-2011
  & 236 % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq13 &\wskip
  & 136 % ASNets
  & 155.4 (10/10) % ASNets (PE)
  & 134 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 208 % LAMA-2011
  & 286 % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq14 &\wskip
  & 158 % ASNets
  & 179 (10/10) % ASNets (PE)
  & 166 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq15 &\wskip
  & 170 % ASNets
  & 219.8 (10/10) % ASNets (PE)
  & 190 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq16 &\wskip
  & 138 % ASNets
  & 156.2 (10/10) % ASNets (PE)
  & 142 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 154 % LAMA-2011
  & 154 % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq17 &\wskip
  & 168 % ASNets
  & 207.8 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 172 % LAMA-2011
  & 172 % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq18 &\wskip
  & 160 % ASNets
  & 201.4 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq19 &\wskip
  & 148 % ASNets
  & 197.4 (10/10) % ASNets (PE)
  & 152 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq2 &\wskip
  & 166 % ASNets
  & 199.8 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq20 &\wskip
  & 152 % ASNets
  & 169.8 (10/10) % ASNets (PE)
  & 156 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 154 % LAMA-2011
  & 154 % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq3 &\wskip
  & 164 % ASNets
  & 198 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 216 % LAMA-2011
  & 240 % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq4 &\wskip
  & 160 % ASNets
  & 185 (10/10) % ASNets (PE)
  & 162 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq5 &\wskip
  & 158 % ASNets
  & 182.6 (10/10) % ASNets (PE)
  & 170 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 240 % LAMA-2011
  & 278 % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq6 &\wskip
  & 134 % ASNets
  & 155.6 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 202 % LAMA-2011
  & 202 % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq7 &\wskip
  & 162 % ASNets
  & 182.6 (10/10) % ASNets (PE)
  & 160 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq8 &\wskip
  & 154 % ASNets
  & 182.2 (10/10) % ASNets (PE)
  & 158 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
blocks-nblk50-seed1184714140-seq9 &\wskip
  & 184 % ASNets
  & 237 (10/10) % ASNets (PE)
  & 188 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\


==> results/det-figures/gold-miner.tex <==
% ASNets & ASNets (PE) & ASNets (no h.) & A* (adm.) & A* (inadm.) & GBF (adm.) & LAMA-2011 & LAMA-first \\
gold-miner-typed-7x7-s70 &\wskip
  & 43 % ASNets
  & 110.4 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 98 &\wskip % GBF (adm.)
  & 45 % LAMA-2011
  & 98 % LAMA-first
  \\
gold-miner-typed-7x7-s71 &\wskip
  & 29 % ASNets
  & 29.5 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & 28 % A* (adm.)
  & 28 &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 28 % LAMA-2011
  & 100 % LAMA-first
  \\
gold-miner-typed-7x7-s72 &\wskip
  & 29 % ASNets
  & 28.7 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & 28 % A* (adm.)
  & 28 &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 28 % LAMA-2011
  & 155 % LAMA-first
  \\
gold-miner-typed-8x8-s80 &\wskip
  & 42 % ASNets
  & 45.8 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 248 % LAMA-2011
  & 248 % LAMA-first
  \\
gold-miner-typed-8x8-s81 &\wskip
  & 36 % ASNets
  & 36.1 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
gold-miner-typed-8x8-s82 &\wskip
  & 40 % ASNets
  & 40.2 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 40 % LAMA-2011
  & 51 % LAMA-first
  \\
gold-miner-typed-9x9-s90 &\wskip
  & 42 % ASNets
  & 45.7 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 42 % LAMA-2011
  & 101 % LAMA-first
  \\
gold-miner-typed-9x9-s91 &\wskip
  & 39 % ASNets
  & 38.3 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 207 % LAMA-2011
  & 207 % LAMA-first
  \\
gold-miner-typed-9x9-s92 &\wskip
  & 36 % ASNets
  & 36.6 (8/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & 36 % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 36 % LAMA-2011
  & 118 % LAMA-first
  \\
gold-miner-typed-10x10-s100 &\wskip
  & 43 % ASNets
  & 43.2 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 259 % LAMA-2011
  & 259 % LAMA-first
  \\
gold-miner-typed-10x10-s101 &\wskip
  & - % ASNets
  & 74.2 (4/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
gold-miner-typed-10x10-s102 &\wskip
  & 38 % ASNets
  & 38.6 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 235 % LAMA-2011
  & 235 % LAMA-first
  \\
gold-miner-typed-13x13-s130 &\wskip
  & 77 % ASNets
  & 83 (2/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
gold-miner-typed-13x13-s131 &\wskip
  & - % ASNets
  & 104.4 (8/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
gold-miner-typed-13x13-s132 &\wskip
  & 64 % ASNets
  & 65.1 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
gold-miner-typed-16x16-s160 &\wskip
  & 71 % ASNets
  & 70.8 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
gold-miner-typed-16x16-s161 &\wskip
  & 83 % ASNets
  & 85.6 (7/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
gold-miner-typed-16x16-s162 &\wskip
  & 75 % ASNets
  & 76.3 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
gold-miner-typed-19x19-s190 &\wskip
  & 89 % ASNets
  & 90.2 (8/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
gold-miner-typed-19x19-s191 &\wskip
  & 80 % ASNets
  & 80.4 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
gold-miner-typed-19x19-s192 &\wskip
  & 103 % ASNets
  & 111 (5/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\


==> results/det-figures/matching-bw.tex <==
% ASNets & ASNets (PE) & ASNets (no h.) & A* (adm.) & A* (inadm.) & GBF (adm.) & LAMA-2011 & LAMA-first \\
mbw-b15-t1-s717 &\wskip
  & 52 % ASNets
  & 59.2 (8/10) % ASNets (PE)
  & 54 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 104 &\wskip % GBF (adm.)
  & 52 % LAMA-2011
  & 142 % LAMA-first
  \\
mbw-b15-t3-s484 &\wskip
  & 38 % ASNets
  & 50.7 (6/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & 38 &\wskip % A* (inadm.)
  & 94 &\wskip % GBF (adm.)
  & 38 % LAMA-2011
  & 78 % LAMA-first
  \\
mbw-b15-t3-s961 &\wskip
  & 42 % ASNets
  & 57 (10/10) % ASNets (PE)
  & 46 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & 38 &\wskip % A* (inadm.)
  & 66 &\wskip % GBF (adm.)
  & 38 % LAMA-2011
  & 72 % LAMA-first
  \\
mbw-b20-t1-s1244 &\wskip
  & 68 % ASNets
  & 87.7 (6/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 292 &\wskip % GBF (adm.)
  & 82 % LAMA-2011
  & 114 % LAMA-first
  \\
mbw-b20-t4-s1749 &\wskip
  & 60 % ASNets
  & 70.9 (9/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 136 &\wskip % GBF (adm.)
  & 68 % LAMA-2011
  & 104 % LAMA-first
  \\
mbw-b20-t4-s1830 &\wskip
  & 56 % ASNets
  & 70 (6/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 102 &\wskip % GBF (adm.)
  & 68 % LAMA-2011
  & 140 % LAMA-first
  \\
mbw-b25-t1-s1727 &\wskip
  & 98 % ASNets
  & 135.4 (7/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 116 % LAMA-2011
  & 214 % LAMA-first
  \\
mbw-b25-t2-s1558 &\wskip
  & 90 % ASNets
  & 106.9 (9/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 106 % LAMA-2011
  & 212 % LAMA-first
  \\
mbw-b25-t5-s888 &\wskip
  & 66 % ASNets
  & 101 (9/10) % ASNets (PE)
  & 64 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b30-t1-s1641 &\wskip
  & 172 % ASNets
  & 150.8 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b30-t5-s1551 &\wskip
  & 258 % ASNets
  & 122.8 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b30-t9-s1824 &\wskip
  & 74 % ASNets
  & 99.5 (10/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 86 % LAMA-2011
  & 126 % LAMA-first
  \\
mbw-b35-t1-s463 &\wskip
  & 162 % ASNets
  & 186.7 (9/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b35-t5-s766 &\wskip
  & 138 % ASNets
  & 165.4 (7/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 140 % LAMA-2011
  & 156 % LAMA-first
  \\
mbw-b35-t8-s688 &\wskip
  & 100 % ASNets
  & 123.6 (9/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b40-t1-s1766 &\wskip
  & 178 % ASNets
  & 208.6 (10/10) % ASNets (PE)
  & 158 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b40-t10-s305 &\wskip
  & 110 % ASNets
  & 133.2 (6/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b40-t6-s1705 &\wskip
  & 108 % ASNets
  & 162.3 (6/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b45-t1-s931 &\wskip
  & 204 % ASNets
  & 269.2 (5/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b45-t2-s782 &\wskip
  & 182 % ASNets
  & 230 (5/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b45-t6-s1396 &\wskip
  & 156 % ASNets
  & 220.2 (8/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b50-t1-s1530 &\wskip
  & - % ASNets
  & 280 (2/10) % ASNets (PE)
  & 210 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b50-t4-s179 &\wskip
  & 270 % ASNets
  & 243.7 (6/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b50-t7-s963 &\wskip
  & 156 % ASNets
  & 244.3 (6/10) % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 180 % LAMA-2011
  & 208 % LAMA-first
  \\
mbw-b55-t1-s992 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b55-t13-s653 &\wskip
  & 146 % ASNets
  & 219 (9/10) % ASNets (PE)
  & 152 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b55-t7-s1529 &\wskip
  & 206 % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b60-t1-s842 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b60-t7-s124 &\wskip
  & 184 % ASNets
  & - % ASNets (PE)
  & 206 &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\
mbw-b60-t7-s261 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no h.)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & - % LAMA-2011
  & - % LAMA-first
  \\


==> results/det-figures/n-puzzle.tex <==
% ASNets & ASNets (PE) \\
n-puzzle-target-4x4-01-n-puzzle-testing-target-typed-n-puzzle-target-4x4-01-typed &\wskip
  & - % ASNets
  & 157 % ASNets (PE)
  \\
n-puzzle-target-4x4-02-n-puzzle-testing-target-typed-n-puzzle-target-4x4-02-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-4x4-03-n-puzzle-testing-target-typed-n-puzzle-target-4x4-03-typed &\wskip
  & - % ASNets
  & 197 % ASNets (PE)
  \\
n-puzzle-target-4x4-04-n-puzzle-testing-target-typed-n-puzzle-target-4x4-04-typed &\wskip
  & - % ASNets
  & 207 % ASNets (PE)
  \\
n-puzzle-target-4x4-05-n-puzzle-testing-target-typed-n-puzzle-target-4x4-05-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-01-n-puzzle-testing-target-typed-n-puzzle-target-5x5-01-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-02-n-puzzle-testing-target-typed-n-puzzle-target-5x5-02-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-03-n-puzzle-testing-target-typed-n-puzzle-target-5x5-03-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-04-n-puzzle-testing-target-typed-n-puzzle-target-5x5-04-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-05-n-puzzle-testing-target-typed-n-puzzle-target-5x5-05-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-06-n-puzzle-testing-target-typed-n-puzzle-target-5x5-06-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-07-n-puzzle-testing-target-typed-n-puzzle-target-5x5-07-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-08-n-puzzle-testing-target-typed-n-puzzle-target-5x5-08-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-09-n-puzzle-testing-target-typed-n-puzzle-target-5x5-09-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-10-n-puzzle-testing-target-typed-n-puzzle-target-5x5-10-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-11-n-puzzle-testing-target-typed-n-puzzle-target-5x5-11-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-12-n-puzzle-testing-target-typed-n-puzzle-target-5x5-12-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-13-n-puzzle-testing-target-typed-n-puzzle-target-5x5-13-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-14-n-puzzle-testing-target-typed-n-puzzle-target-5x5-14-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-5x5-15-n-puzzle-testing-target-typed-n-puzzle-target-5x5-15-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-6x6-01-n-puzzle-testing-target-typed-n-puzzle-target-6x6-01-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-6x6-02-n-puzzle-testing-target-typed-n-puzzle-target-6x6-02-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-6x6-03-n-puzzle-testing-target-typed-n-puzzle-target-6x6-03-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-6x6-04-n-puzzle-testing-target-typed-n-puzzle-target-6x6-04-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-6x6-05-n-puzzle-testing-target-typed-n-puzzle-target-6x6-05-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-7x7-01-n-puzzle-testing-target-typed-n-puzzle-target-7x7-01-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-7x7-02-n-puzzle-testing-target-typed-n-puzzle-target-7x7-02-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-7x7-03-n-puzzle-testing-target-typed-n-puzzle-target-7x7-03-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-7x7-04-n-puzzle-testing-target-typed-n-puzzle-target-7x7-04-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\
n-puzzle-target-7x7-05-n-puzzle-testing-target-typed-n-puzzle-target-7x7-05-typed &\wskip
  & - % ASNets
  & - % ASNets (PE)
  \\


==> results/det-figures/parking.tex <==
% ASNets & ASNets (PE) & ASNets (no LM) & A* (adm.) & A* (inadm.) & GBF (adm.) & LAMA-2011 & LAMA-first \\
parking-c10-05 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 66 &\wskip % GBF (adm.)
  & 27 % LAMA-2011
  & 49 % LAMA-first
  \\
parking-c10-07 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 59 &\wskip % GBF (adm.)
  & 29 % LAMA-2011
  & 59 % LAMA-first
  \\
parking-c10-08 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 39 &\wskip % A* (inadm.)
  & 48 &\wskip % GBF (adm.)
  & 28 % LAMA-2011
  & 53 % LAMA-first
  \\
parking-c10-09 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 56 &\wskip % GBF (adm.)
  & 29 % LAMA-2011
  & 53 % LAMA-first
  \\
parking-c10-10 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 37 &\wskip % A* (inadm.)
  & 57 &\wskip % GBF (adm.)
  & 30 % LAMA-2011
  & 55 % LAMA-first
  \\
parking-c12-06 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 73 &\wskip % GBF (adm.)
  & 37 % LAMA-2011
  & 76 % LAMA-first
  \\
parking-c12-07 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 47 &\wskip % A* (inadm.)
  & 78 &\wskip % GBF (adm.)
  & 67 % LAMA-2011
  & 57 % LAMA-first
  \\
parking-c12-08 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 80 &\wskip % GBF (adm.)
  & 42 % LAMA-2011
  & 72 % LAMA-first
  \\
parking-c12-09 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 42 &\wskip % A* (inadm.)
  & 73 &\wskip % GBF (adm.)
  & 32 % LAMA-2011
  & 48 % LAMA-first
  \\
parking-c12-10 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 80 &\wskip % GBF (adm.)
  & 38 % LAMA-2011
  & 75 % LAMA-first
  \\
parking-c13-06 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 72 &\wskip % GBF (adm.)
  & 66 % LAMA-2011
  & 68 % LAMA-first
  \\
parking-c13-07 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 90 &\wskip % GBF (adm.)
  & 39 % LAMA-2011
  & 73 % LAMA-first
  \\
parking-c13-08 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 70 &\wskip % GBF (adm.)
  & 62 % LAMA-2011
  & 81 % LAMA-first
  \\
parking-c13-09 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 44 &\wskip % A* (inadm.)
  & 61 &\wskip % GBF (adm.)
  & 57 % LAMA-2011
  & 58 % LAMA-first
  \\
parking-c13-10 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 69 &\wskip % GBF (adm.)
  & 37 % LAMA-2011
  & 77 % LAMA-first
  \\
parking-c15-01 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 79 % LAMA-2011
  & 83 % LAMA-first
  \\
parking-c15-02 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 52 % LAMA-2011
  & 98 % LAMA-first
  \\
parking-c15-03 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 51 &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 58 % LAMA-2011
  & 93 % LAMA-first
  \\
parking-c15-04 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 68 &\wskip % GBF (adm.)
  & 78 % LAMA-2011
  & 74 % LAMA-first
  \\
parking-c15-05 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 67 % LAMA-2011
  & 88 % LAMA-first
  \\
parking-c15-06 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 51 % LAMA-2011
  & 95 % LAMA-first
  \\
parking-c15-07 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 84 % LAMA-2011
  & 84 % LAMA-first
  \\
parking-c15-08 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 65 % LAMA-2011
  & 84 % LAMA-first
  \\
parking-c15-09 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 70 % LAMA-2011
  & 59 % LAMA-first
  \\
parking-c15-10 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 53 % LAMA-2011
  & 67 % LAMA-first
  \\
parking-c20-01 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 63 % LAMA-2011
  & 122 % LAMA-first
  \\
parking-c20-02 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 90 % LAMA-2011
  & 103 % LAMA-first
  \\
parking-c20-03 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 62 % LAMA-2011
  & 115 % LAMA-first
  \\
parking-c20-04 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 97 % LAMA-2011
  & 128 % LAMA-first
  \\
parking-c20-05 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 63 % LAMA-2011
  & 91 % LAMA-first
  \\


==> results/det-figures/sokoban.tex <==
% ASNets & ASNets (PE) & ASNets (no LM) & A* (adm.) & A* (inadm.) & GBF (adm.) & LAMA-2011 & LAMA-first \\
sokoban-n09-b03-w04-01 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 51 % A* (adm.)
  & 51 &\wskip % A* (inadm.)
  & 67 &\wskip % GBF (adm.)
  & 51 % LAMA-2011
  & 99 % LAMA-first
  \\
sokoban-n09-b03-w04-02 &\wskip
  & - % ASNets
  & 90 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 68 % A* (adm.)
  & 68 &\wskip % A* (inadm.)
  & 160 &\wskip % GBF (adm.)
  & 68 % LAMA-2011
  & 112 % LAMA-first
  \\
sokoban-n09-b03-w04-03 &\wskip
  & - % ASNets
  & 126.3 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 57 % A* (adm.)
  & 57 &\wskip % A* (inadm.)
  & 89 &\wskip % GBF (adm.)
  & 57 % LAMA-2011
  & 79 % LAMA-first
  \\
sokoban-n09-b03-w04-04 &\wskip
  & - % ASNets
  & 75 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 59 % A* (adm.)
  & 59 &\wskip % A* (inadm.)
  & 85 &\wskip % GBF (adm.)
  & 59 % LAMA-2011
  & 71 % LAMA-first
  \\
sokoban-n09-b03-w04-05 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 62 % A* (adm.)
  & 64 &\wskip % A* (inadm.)
  & 94 &\wskip % GBF (adm.)
  & 62 % LAMA-2011
  & 150 % LAMA-first
  \\
sokoban-n09-b03-w04-06 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 56 % A* (adm.)
  & 56 &\wskip % A* (inadm.)
  & 92 &\wskip % GBF (adm.)
  & 56 % LAMA-2011
  & 104 % LAMA-first
  \\
sokoban-n09-b03-w04-07 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 68 % A* (adm.)
  & 68 &\wskip % A* (inadm.)
  & 160 &\wskip % GBF (adm.)
  & 68 % LAMA-2011
  & 112 % LAMA-first
  \\
sokoban-n09-b03-w04-08 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 59 % A* (adm.)
  & 59 &\wskip % A* (inadm.)
  & 85 &\wskip % GBF (adm.)
  & 59 % LAMA-2011
  & 69 % LAMA-first
  \\
sokoban-n09-b03-w04-09 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 59 % A* (adm.)
  & 59 &\wskip % A* (inadm.)
  & 99 &\wskip % GBF (adm.)
  & 59 % LAMA-2011
  & 81 % LAMA-first
  \\
sokoban-n09-b03-w04-10 &\wskip
  & - % ASNets
  & 76 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 55 % A* (adm.)
  & 55 &\wskip % A* (inadm.)
  & 99 &\wskip % GBF (adm.)
  & 55 % LAMA-2011
  & 71 % LAMA-first
  \\
sokoban-n09-b04-w04-01 &\wskip
  & - % ASNets
  & 132 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 74 &\wskip % A* (inadm.)
  & 144 &\wskip % GBF (adm.)
  & 74 % LAMA-2011
  & 116 % LAMA-first
  \\
sokoban-n09-b04-w04-02 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 187 &\wskip % GBF (adm.)
  & 83 % LAMA-2011
  & 179 % LAMA-first
  \\
sokoban-n09-b04-w04-03 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 134 &\wskip % GBF (adm.)
  & 76 % LAMA-2011
  & 108 % LAMA-first
  \\
sokoban-n09-b04-w04-04 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 138 &\wskip % GBF (adm.)
  & 78 % LAMA-2011
  & 200 % LAMA-first
  \\
sokoban-n09-b04-w04-05 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 277 &\wskip % GBF (adm.)
  & 83 % LAMA-2011
  & 163 % LAMA-first
  \\
sokoban-n09-b04-w04-06 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 149 &\wskip % GBF (adm.)
  & 75 % LAMA-2011
  & 111 % LAMA-first
  \\
sokoban-n09-b04-w04-07 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 227 &\wskip % GBF (adm.)
  & 93 % LAMA-2011
  & 141 % LAMA-first
  \\
sokoban-n09-b04-w04-08 &\wskip
  & - % ASNets
  & 103 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 153 &\wskip % GBF (adm.)
  & 79 % LAMA-2011
  & 95 % LAMA-first
  \\
sokoban-n09-b04-w04-09 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 255 &\wskip % GBF (adm.)
  & 81 % LAMA-2011
  & 179 % LAMA-first
  \\
sokoban-n09-b04-w04-10 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 159 &\wskip % GBF (adm.)
  & 77 % LAMA-2011
  & 141 % LAMA-first
  \\
sokoban-n09-b04-w04-11 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 139 &\wskip % GBF (adm.)
  & 69 % LAMA-2011
  & 77 % LAMA-first
  \\
sokoban-n09-b04-w04-12 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 155 &\wskip % GBF (adm.)
  & 87 % LAMA-2011
  & 129 % LAMA-first
  \\
sokoban-n09-b04-w04-13 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 292 &\wskip % GBF (adm.)
  & 82 % LAMA-2011
  & 128 % LAMA-first
  \\
sokoban-n09-b04-w04-14 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 156 &\wskip % GBF (adm.)
  & 86 % LAMA-2011
  & 132 % LAMA-first
  \\
sokoban-n09-b04-w04-15 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 166 &\wskip % GBF (adm.)
  & 84 % LAMA-2011
  & 174 % LAMA-first
  \\
sokoban-n09-b04-w04-16 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 134 &\wskip % GBF (adm.)
  & 84 % LAMA-2011
  & 138 % LAMA-first
  \\
sokoban-n09-b04-w04-17 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 149 &\wskip % GBF (adm.)
  & 79 % LAMA-2011
  & 245 % LAMA-first
  \\
sokoban-n09-b04-w04-18 &\wskip
  & - % ASNets
  & 79 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 67 &\wskip % A* (inadm.)
  & 127 &\wskip % GBF (adm.)
  & 67 % LAMA-2011
  & 83 % LAMA-first
  \\
sokoban-n09-b04-w04-19 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 73 &\wskip % A* (inadm.)
  & 155 &\wskip % GBF (adm.)
  & 73 % LAMA-2011
  & 89 % LAMA-first
  \\
sokoban-n09-b04-w04-20 &\wskip
  & - % ASNets
  & 125 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 127 &\wskip % GBF (adm.)
  & 73 % LAMA-2011
  & 93 % LAMA-first
  \\


==> results/prob-figures/cn-0.tex <==
% ASNets & ASNets (PE) & ASNets (adm.) & ASNets (no h.) & LRTDP & LRTDP (adm.) & SSiPP & SSiPP (adm.) \\
cosanostra-n6 &\wskip
  & \makecell{30/30 \\ (22.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (22.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (22.0 $\pm$ 0)} % ASNets (adm.)
  & \makecell{30/30 \\ (22.0 $\pm$ 0)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (22.0 $\pm$ 0)} % LRTDP
  & \makecell{30/30 \\ (22.0 $\pm$ 0)} &\wskip % LRTDP (adm.)
  & \makecell{30/30 \\ (22.0 $\pm$ 0)} % SSiPP
  & \makecell{30/30 \\ (22.0 $\pm$ 0)} % SSiPP (adm.)
  \\
cosanostra-n7 &\wskip
  & \makecell{30/30 \\ (25.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (25.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (25.0 $\pm$ 0)} % ASNets (adm.)
  & \makecell{30/30 \\ (25.0 $\pm$ 0)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (25.0 $\pm$ 0)} % LRTDP
  & \makecell{30/30 \\ (25.0 $\pm$ 0)} &\wskip % LRTDP (adm.)
  & \makecell{30/30 \\ (25.0 $\pm$ 0)} % SSiPP
  & \makecell{30/30 \\ (25.0 $\pm$ 0)} % SSiPP (adm.)
  \\
cosanostra-n8 &\wskip
  & \makecell{30/30 \\ (28.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (28.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (28.0 $\pm$ 0)} % ASNets (adm.)
  & \makecell{30/30 \\ (28.0 $\pm$ 0)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (28.0 $\pm$ 0)} % LRTDP
  & \makecell{30/30 \\ (28.0 $\pm$ 0)} &\wskip % LRTDP (adm.)
  & \makecell{30/30 \\ (28.0 $\pm$ 0)} % SSiPP
  & \makecell{30/30 \\ (28.0 $\pm$ 0)} % SSiPP (adm.)
  \\
cosanostra-n9 &\wskip
  & \makecell{30/30 \\ (31.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (31.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (31.0 $\pm$ 0)} % ASNets (adm.)
  & \makecell{30/30 \\ (31.0 $\pm$ 0)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (31.0 $\pm$ 0)} % LRTDP
  & \makecell{30/30 \\ (31.0 $\pm$ 0)} &\wskip % LRTDP (adm.)
  & \makecell{30/30 \\ (31.0 $\pm$ 0)} % SSiPP
  & \makecell{30/30 \\ (31.0 $\pm$ 0)} % SSiPP (adm.)
  \\
cosanostra-n10 &\wskip
  & \makecell{30/30 \\ (34.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (34.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (34.0 $\pm$ 0)} % ASNets (adm.)
  & \makecell{30/30 \\ (34.0 $\pm$ 0)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (34.0 $\pm$ 0)} % LRTDP
  & \makecell{11/30 \\ (34.0 $\pm$ 0)} &\wskip % LRTDP (adm.)
  & \makecell{30/30 \\ (34.0 $\pm$ 0)} % SSiPP
  & \makecell{11/30 \\ (34.0 $\pm$ 0)} % SSiPP (adm.)
  \\
cosanostra-n11 &\wskip
  & \makecell{30/30 \\ (37.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (37.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (37.0 $\pm$ 0)} % ASNets (adm.)
  & \makecell{30/30 \\ (37.0 $\pm$ 0)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (37.0 $\pm$ 0)} % LRTDP
  & \makecell{4/30 \\ (37.0 $\pm$ 0)} &\wskip % LRTDP (adm.)
  & \makecell{23/30 \\ (37.0 $\pm$ 0)} % SSiPP
  & \makecell{4/30 \\ (37.0 $\pm$ 0)} % SSiPP (adm.)
  \\
cosanostra-n12 &\wskip
  & \makecell{30/30 \\ (40.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (40.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (40.0 $\pm$ 0)} % ASNets (adm.)
  & \makecell{30/30 \\ (40.0 $\pm$ 0)} &\wskip % ASNets (no h.)
  & \makecell{13/30 \\ (40.0 $\pm$ 0)} % LRTDP
  & \makecell{1/30 \\ (40.0)} &\wskip % LRTDP (adm.)
  & \makecell{10/30 \\ (40.0 $\pm$ 0)} % SSiPP
  & \makecell{2/30 \\ (40.0 $\pm$ 0)} % SSiPP (adm.)
  \\
cosanostra-n13 &\wskip
  & \makecell{30/30 \\ (43.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (43.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (43.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & \makecell{6/30 \\ (43.0 $\pm$ 0)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{4/30 \\ (43.0 $\pm$ 0)} % SSiPP
  & - % SSiPP (adm.)
  \\
cosanostra-n14 &\wskip
  & \makecell{30/30 \\ (46.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (46.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (46.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & \makecell{2/30 \\ (46.0 $\pm$ 0)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{2/30 \\ (46.0 $\pm$ 0)} % SSiPP
  & - % SSiPP (adm.)
  \\
cosanostra-n15 &\wskip
  & \makecell{30/30 \\ (49.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (49.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (49.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & \makecell{1/30 \\ (49.0)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
cosanostra-n20 &\wskip
  & \makecell{30/30 \\ (64.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (64.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (64.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
cosanostra-n25 &\wskip
  & \makecell{30/30 \\ (79.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (79.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (79.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
cosanostra-n30 &\wskip
  & \makecell{30/30 \\ (94.0 $\pm$ 0)} % ASNets
  & \makecell{29/30 \\ (94.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (94.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
cosanostra-n35 &\wskip
  & \makecell{30/30 \\ (109.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (109.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (109.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
cosanostra-n40 &\wskip
  & \makecell{30/30 \\ (124.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (124.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (124.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
cosanostra-n45 &\wskip
  & \makecell{30/30 \\ (139.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (139.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (139.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
cosanostra-n50 &\wskip
  & \makecell{30/30 \\ (154.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (154.0 $\pm$ 0)} % ASNets (PE)
  & \makecell{30/30 \\ (154.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\


==> results/prob-figures/exbw-0.tex <==
% ASNets & ASNets (PE) & ASNets (adm.) & ASNets (no h.) & LRTDP & LRTDP (adm.) & SSiPP & SSiPP (adm.) \\
ex-bw-b11-s0 &\wskip
  & \makecell{15/30 \\ (28.0 $\pm$ 0)} % ASNets
  & \makecell{9/30 \\ (36.7 $\pm$ 9.8)} % ASNets (PE)
  & \makecell{15/30 \\ (28.0 $\pm$ 0)} % ASNets (adm.)
  & \makecell{17/30 \\ (28.9 $\pm$ 0.5)} &\wskip % ASNets (no h.)
  & \makecell{21/30 \\ (44.4 $\pm$ 9.4)} % LRTDP
  & \makecell{28/30 \\ (45.0 $\pm$ 7.3)} &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (32.0)} % SSiPP
  & \makecell{4/30 \\ (66.0 $\pm$ 55.2)} % SSiPP (adm.)
  \\
ex-bw-b11-s1 &\wskip
  & - % ASNets
  & \makecell{3/30 \\ (88.0 $\pm$ 86.2)} % ASNets (PE)
  & - % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & \makecell{4/30 \\ (99.5 $\pm$ 29.7)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & \makecell{1/30 \\ (64.0)} % SSiPP (adm.)
  \\
ex-bw-b11-s2 &\wskip
  & \makecell{16/30 \\ (26.0 $\pm$ 0)} % ASNets
  & \makecell{17/30 \\ (30.2 $\pm$ 1.6)} % ASNets (PE)
  & \makecell{16/30 \\ (26.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & \makecell{23/30 \\ (28.4 $\pm$ 1.1)} % LRTDP
  & \makecell{2/30 \\ (24.0 $\pm$ 0)} &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (28.0)} % SSiPP
  & \makecell{1/30 \\ (24.0)} % SSiPP (adm.)
  \\
ex-bw-b12-s0 &\wskip
  & \makecell{29/30 \\ (26.0 $\pm$ 0)} % ASNets
  & \makecell{30/30 \\ (26.3 $\pm$ 0.3)} % ASNets (PE)
  & \makecell{29/30 \\ (26.0 $\pm$ 0)} % ASNets (adm.)
  & \makecell{29/30 \\ (26.0 $\pm$ 0)} &\wskip % ASNets (no h.)
  & \makecell{29/30 \\ (28.2 $\pm$ 1.5)} % LRTDP
  & \makecell{9/30 \\ (26.0 $\pm$ 0)} &\wskip % LRTDP (adm.)
  & \makecell{28/30 \\ (27.7 $\pm$ 0.9)} % SSiPP
  & \makecell{13/30 \\ (26.9 $\pm$ 1.2)} % SSiPP (adm.)
  \\
ex-bw-b12-s1 &\wskip
  & - % ASNets
  & \makecell{4/30 \\ (65.0 $\pm$ 32.9)} % ASNets (PE)
  & \makecell{3/30 \\ (56.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & \makecell{1/30 \\ (52.0)} % LRTDP
  & \makecell{6/30 \\ (67.0 $\pm$ 33.0)} &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b12-s2 &\wskip
  & - % ASNets
  & \makecell{5/30 \\ (76.4 $\pm$ 32.1)} % ASNets (PE)
  & \makecell{5/30 \\ (42.4 $\pm$ 13.8)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & \makecell{1/30 \\ (42.0)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b13-s0 &\wskip
  & \makecell{26/30 \\ (25.6 $\pm$ 1.1)} % ASNets
  & \makecell{24/30 \\ (27.4 $\pm$ 1.5)} % ASNets (PE)
  & \makecell{29/30 \\ (25.2 $\pm$ 0.4)} % ASNets (adm.)
  & \makecell{27/30 \\ (25.3 $\pm$ 0.4)} &\wskip % ASNets (no h.)
  & \makecell{27/30 \\ (27.9 $\pm$ 0.8)} % LRTDP
  & \makecell{26/30 \\ (24.0 $\pm$ 0)} &\wskip % LRTDP (adm.)
  & \makecell{27/30 \\ (28.1 $\pm$ 1.1)} % SSiPP
  & \makecell{21/30 \\ (24.0 $\pm$ 0)} % SSiPP (adm.)
  \\
ex-bw-b13-s1 &\wskip
  & - % ASNets
  & \makecell{2/30 \\ (56.0 $\pm$ 203.3)} % ASNets (PE)
  & \makecell{7/30 \\ (60.3 $\pm$ 23.1)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & \makecell{9/30 \\ (79.3 $\pm$ 22.6)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b13-s2 &\wskip
  & \makecell{11/30 \\ (58.7 $\pm$ 10.2)} % ASNets
  & \makecell{2/30 \\ (57.0 $\pm$ 63.5)} % ASNets (PE)
  & \makecell{11/30 \\ (49.1 $\pm$ 12.9)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & \makecell{14/30 \\ (63.1 $\pm$ 15.9)} % LRTDP
  & \makecell{1/30 \\ (82.0)} &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b14-s0 &\wskip
  & - % ASNets
  & \makecell{5/30 \\ (64.8 $\pm$ 17.3)} % ASNets (PE)
  & - % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b14-s1 &\wskip
  & - % ASNets
  & \makecell{6/30 \\ (62.0 $\pm$ 20.7)} % ASNets (PE)
  & \makecell{15/30 \\ (34.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b14-s2 &\wskip
  & \makecell{12/30 \\ (38.0 $\pm$ 0)} % ASNets
  & \makecell{12/30 \\ (40.7 $\pm$ 1.9)} % ASNets (PE)
  & \makecell{14/30 \\ (36.0 $\pm$ 0)} % ASNets (adm.)
  & \makecell{12/30 \\ (38.0 $\pm$ 0)} &\wskip % ASNets (no h.)
  & \makecell{10/30 \\ (55.4 $\pm$ 10.1)} % LRTDP
  & \makecell{1/30 \\ (46.0)} &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (80.0)} % SSiPP
  & \makecell{1/30 \\ (68.0)} % SSiPP (adm.)
  \\
ex-bw-b15-s0 &\wskip
  & \makecell{6/30 \\ (41.3 $\pm$ 1.1)} % ASNets
  & \makecell{9/30 \\ (45.8 $\pm$ 3.0)} % ASNets (PE)
  & \makecell{7/30 \\ (48.3 $\pm$ 4.9)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b15-s1 &\wskip
  & \makecell{6/30 \\ (69.3 $\pm$ 18.7)} % ASNets
  & \makecell{2/30 \\ (61.0 $\pm$ 38.1)} % ASNets (PE)
  & \makecell{3/30 \\ (56.0 $\pm$ 9.9)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b15-s2 &\wskip
  & \makecell{18/30 \\ (56.7 $\pm$ 5.8)} % ASNets
  & \makecell{14/30 \\ (54.1 $\pm$ 16.6)} % ASNets (PE)
  & \makecell{13/30 \\ (51.2 $\pm$ 3.5)} % ASNets (adm.)
  & \makecell{14/30 \\ (36.0 $\pm$ 0)} &\wskip % ASNets (no h.)
  & \makecell{5/30 \\ (73.6 $\pm$ 28.7)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (66.0)} % SSiPP
  & \makecell{1/30 \\ (96.0)} % SSiPP (adm.)
  \\
ex-bw-b16-s0 &\wskip
  & - % ASNets
  & \makecell{13/30 \\ (69.8 $\pm$ 17.7)} % ASNets (PE)
  & \makecell{14/30 \\ (53.0 $\pm$ 12.2)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b16-s1 &\wskip
  & \makecell{4/30 \\ (61.0 $\pm$ 20.2)} % ASNets
  & \makecell{4/30 \\ (69.0 $\pm$ 19.7)} % ASNets (PE)
  & \makecell{6/30 \\ (46.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (46.0)} % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b16-s2 &\wskip
  & \makecell{1/30 \\ (78.0)} % ASNets
  & \makecell{3/30 \\ (70.7 $\pm$ 30.4)} % ASNets (PE)
  & \makecell{3/30 \\ (62.0 $\pm$ 8.6)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b17-s0 &\wskip
  & \makecell{1/30 \\ (76.0)} % ASNets
  & \makecell{5/30 \\ (62.4 $\pm$ 15.4)} % ASNets (PE)
  & \makecell{3/30 \\ (52.7 $\pm$ 20.1)} % ASNets (adm.)
  & \makecell{3/30 \\ (80.0 $\pm$ 117.5)} &\wskip % ASNets (no h.)
  & \makecell{1/30 \\ (42.0)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b17-s1 &\wskip
  & \makecell{7/30 \\ (67.4 $\pm$ 30.3)} % ASNets
  & \makecell{2/30 \\ (66.0 $\pm$ 76.2)} % ASNets (PE)
  & \makecell{4/30 \\ (101.0 $\pm$ 84.9)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b17-s2 &\wskip
  & \makecell{1/30 \\ (64.0)} % ASNets
  & \makecell{2/30 \\ (93.0 $\pm$ 165.2)} % ASNets (PE)
  & - % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b18-s0 &\wskip
  & - % ASNets
  & \makecell{2/30 \\ (76.0 $\pm$ 25.4)} % ASNets (PE)
  & \makecell{4/30 \\ (70.5 $\pm$ 8.0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b18-s1 &\wskip
  & \makecell{2/30 \\ (53.0 $\pm$ 12.7)} % ASNets
  & \makecell{4/30 \\ (71.5 $\pm$ 22.0)} % ASNets (PE)
  & \makecell{2/30 \\ (72.0 $\pm$ 25.4)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b18-s2 &\wskip
  & - % ASNets
  & \makecell{1/30 \\ (104.0)} % ASNets (PE)
  & - % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b19-s0 &\wskip
  & - % ASNets
  & \makecell{8/30 \\ (99.0 $\pm$ 13.3)} % ASNets (PE)
  & \makecell{2/30 \\ (83.0 $\pm$ 368.5)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b19-s1 &\wskip
  & - % ASNets
  & \makecell{1/30 \\ (96.0)} % ASNets (PE)
  & - % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b19-s2 &\wskip
  & \makecell{10/30 \\ (57.8 $\pm$ 1.3)} % ASNets
  & \makecell{8/30 \\ (63.2 $\pm$ 4.6)} % ASNets (PE)
  & \makecell{17/30 \\ (52.0 $\pm$ 0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b20-s0 &\wskip
  & \makecell{1/30 \\ (70.0)} % ASNets
  & \makecell{2/30 \\ (78.0 $\pm$ 254.1)} % ASNets (PE)
  & \makecell{6/30 \\ (79.7 $\pm$ 27.1)} % ASNets (adm.)
  & \makecell{4/30 \\ (81.5 $\pm$ 18.8)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b20-s1 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & \makecell{5/30 \\ (76.0 $\pm$ 12.0)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
ex-bw-b20-s2 &\wskip
  & - % ASNets
  & \makecell{1/30 \\ (86.0)} % ASNets (PE)
  & - % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\


==> results/prob-figures/pbw-0.tex <==
% ASNets & ASNets (PE) & ASNets (adm.) & ASNets (no h.) & LRTDP & LRTDP (adm.) & SSiPP & SSiPP (adm.) \\
prob-bw-b15-s1 &\wskip
  & \makecell{30/30 \\ (49.4 $\pm$ 2.2)} % ASNets
  & \makecell{30/30 \\ (53.8 $\pm$ 2.7)} % ASNets (PE)
  & \makecell{30/30 \\ (48.9 $\pm$ 1.8)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (52.9 $\pm$ 2.5)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{20/30 \\ (110.4 $\pm$ 23.0)} % SSiPP
  & \makecell{1/30 \\ (241.0)} % SSiPP (adm.)
  \\
prob-bw-b15-s2 &\wskip
  & \makecell{30/30 \\ (42.2 $\pm$ 2.1)} % ASNets
  & \makecell{30/30 \\ (48.2 $\pm$ 2.8)} % ASNets (PE)
  & \makecell{30/30 \\ (42.8 $\pm$ 2.0)} % ASNets (adm.)
  & \makecell{30/30 \\ (44.2 $\pm$ 2.1)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (48.3 $\pm$ 2.3)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{30/30 \\ (114.1 $\pm$ 21.5)} % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b15-s3 &\wskip
  & \makecell{30/30 \\ (66.0 $\pm$ 2.2)} % ASNets
  & \makecell{30/30 \\ (67.3 $\pm$ 2.2)} % ASNets (PE)
  & \makecell{30/30 \\ (63.8 $\pm$ 2.2)} % ASNets (adm.)
  & \makecell{30/30 \\ (66.0 $\pm$ 2.2)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (74.6 $\pm$ 2.7)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{30/30 \\ (70.7 $\pm$ 3.0)} % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b15-s4 &\wskip
  & \makecell{30/30 \\ (48.6 $\pm$ 2.0)} % ASNets
  & \makecell{30/30 \\ (49.2 $\pm$ 2.0)} % ASNets (PE)
  & \makecell{30/30 \\ (48.4 $\pm$ 2.2)} % ASNets (adm.)
  & \makecell{30/30 \\ (48.6 $\pm$ 2.0)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (58.3 $\pm$ 4.2)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{19/30 \\ (107.9 $\pm$ 20.7)} % SSiPP
  & \makecell{1/30 \\ (168.0)} % SSiPP (adm.)
  \\
prob-bw-b15-s5 &\wskip
  & \makecell{30/30 \\ (52.3 $\pm$ 2.5)} % ASNets
  & \makecell{30/30 \\ (54.6 $\pm$ 2.5)} % ASNets (PE)
  & \makecell{30/30 \\ (46.1 $\pm$ 2.2)} % ASNets (adm.)
  & \makecell{30/30 \\ (54.8 $\pm$ 2.4)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (55.1 $\pm$ 1.5)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{19/30 \\ (140.8 $\pm$ 29.4)} % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b20-s1 &\wskip
  & \makecell{30/30 \\ (73.5 $\pm$ 2.4)} % ASNets
  & \makecell{30/30 \\ (77.1 $\pm$ 3.0)} % ASNets (PE)
  & \makecell{30/30 \\ (73.5 $\pm$ 2.3)} % ASNets (adm.)
  & \makecell{30/30 \\ (72.3 $\pm$ 2.4)} &\wskip % ASNets (no h.)
  & \makecell{12/30 \\ (81.1 $\pm$ 6.9)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (91.0)} % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b20-s2 &\wskip
  & \makecell{30/30 \\ (68.5 $\pm$ 2.7)} % ASNets
  & \makecell{30/30 \\ (76.1 $\pm$ 2.5)} % ASNets (PE)
  & \makecell{30/30 \\ (69.2 $\pm$ 2.3)} % ASNets (adm.)
  & \makecell{30/30 \\ (68.4 $\pm$ 2.6)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (77.0 $\pm$ 2.9)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (79.0)} % SSiPP
  & \makecell{1/30 \\ (89.0)} % SSiPP (adm.)
  \\
prob-bw-b20-s3 &\wskip
  & \makecell{30/30 \\ (68.7 $\pm$ 2.0)} % ASNets
  & \makecell{30/30 \\ (71.0 $\pm$ 3.2)} % ASNets (PE)
  & \makecell{30/30 \\ (68.7 $\pm$ 2.5)} % ASNets (adm.)
  & \makecell{30/30 \\ (69.3 $\pm$ 2.5)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (78.2 $\pm$ 2.6)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{4/30 \\ (74.2 $\pm$ 8.5)} % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b20-s4 &\wskip
  & \makecell{30/30 \\ (76.3 $\pm$ 2.5)} % ASNets
  & \makecell{30/30 \\ (80.3 $\pm$ 2.7)} % ASNets (PE)
  & \makecell{30/30 \\ (73.1 $\pm$ 2.7)} % ASNets (adm.)
  & \makecell{30/30 \\ (76.2 $\pm$ 2.4)} &\wskip % ASNets (no h.)
  & \makecell{28/30 \\ (87.6 $\pm$ 3.9)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (73.0)} % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b20-s5 &\wskip
  & \makecell{30/30 \\ (84.2 $\pm$ 2.4)} % ASNets
  & \makecell{30/30 \\ (84.7 $\pm$ 2.4)} % ASNets (PE)
  & \makecell{30/30 \\ (83.0 $\pm$ 2.8)} % ASNets (adm.)
  & \makecell{30/30 \\ (84.2 $\pm$ 2.4)} &\wskip % ASNets (no h.)
  & \makecell{19/30 \\ (85.4 $\pm$ 3.7)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{12/30 \\ (85.1 $\pm$ 3.2)} % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b25-s1 &\wskip
  & \makecell{30/30 \\ (90.4 $\pm$ 2.7)} % ASNets
  & \makecell{30/30 \\ (101.4 $\pm$ 3.4)} % ASNets (PE)
  & \makecell{30/30 \\ (93.7 $\pm$ 2.5)} % ASNets (adm.)
  & \makecell{30/30 \\ (90.0 $\pm$ 2.7)} &\wskip % ASNets (no h.)
  & \makecell{1/30 \\ (79.0)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{4/30 \\ (135.2 $\pm$ 120.6)} % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b25-s2 &\wskip
  & \makecell{30/30 \\ (90.1 $\pm$ 2.7)} % ASNets
  & \makecell{30/30 \\ (92.7 $\pm$ 2.3)} % ASNets (PE)
  & \makecell{30/30 \\ (88.1 $\pm$ 2.5)} % ASNets (adm.)
  & \makecell{30/30 \\ (89.3 $\pm$ 2.5)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (88.0)} % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b25-s3 &\wskip
  & \makecell{30/30 \\ (84.5 $\pm$ 2.2)} % ASNets
  & \makecell{30/30 \\ (88.8 $\pm$ 3.1)} % ASNets (PE)
  & \makecell{30/30 \\ (77.8 $\pm$ 2.6)} % ASNets (adm.)
  & - &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{2/30 \\ (106.5 $\pm$ 184.2)} % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b25-s4 &\wskip
  & \makecell{30/30 \\ (101.0 $\pm$ 3.1)} % ASNets
  & \makecell{30/30 \\ (100.9 $\pm$ 3.3)} % ASNets (PE)
  & \makecell{30/30 \\ (91.9 $\pm$ 2.9)} % ASNets (adm.)
  & \makecell{30/30 \\ (95.6 $\pm$ 2.6)} &\wskip % ASNets (no h.)
  & \makecell{2/30 \\ (106.0 $\pm$ 76.2)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (162.0)} % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b25-s5 &\wskip
  & \makecell{30/30 \\ (91.7 $\pm$ 2.3)} % ASNets
  & \makecell{30/30 \\ (93.7 $\pm$ 2.5)} % ASNets (PE)
  & \makecell{30/30 \\ (89.4 $\pm$ 2.6)} % ASNets (adm.)
  & \makecell{30/30 \\ (90.5 $\pm$ 2.8)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b30-s1 &\wskip
  & \makecell{30/30 \\ (106.5 $\pm$ 3.4)} % ASNets
  & \makecell{30/30 \\ (116.4 $\pm$ 3.6)} % ASNets (PE)
  & \makecell{30/30 \\ (102.7 $\pm$ 2.5)} % ASNets (adm.)
  & \makecell{30/30 \\ (109.4 $\pm$ 3.0)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b30-s2 &\wskip
  & \makecell{30/30 \\ (101.4 $\pm$ 2.3)} % ASNets
  & \makecell{30/30 \\ (108.5 $\pm$ 3.1)} % ASNets (PE)
  & \makecell{30/30 \\ (103.7 $\pm$ 3.4)} % ASNets (adm.)
  & \makecell{30/30 \\ (106.2 $\pm$ 2.7)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (148.0)} % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b30-s3 &\wskip
  & \makecell{30/30 \\ (111.4 $\pm$ 2.6)} % ASNets
  & \makecell{30/30 \\ (121.9 $\pm$ 3.4)} % ASNets (PE)
  & \makecell{30/30 \\ (110.0 $\pm$ 3.3)} % ASNets (adm.)
  & \makecell{30/30 \\ (111.4 $\pm$ 2.8)} &\wskip % ASNets (no h.)
  & \makecell{1/30 \\ (135.0)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b30-s4 &\wskip
  & \makecell{30/30 \\ (111.5 $\pm$ 3.5)} % ASNets
  & \makecell{30/30 \\ (115.2 $\pm$ 3.8)} % ASNets (PE)
  & \makecell{30/30 \\ (108.6 $\pm$ 2.6)} % ASNets (adm.)
  & \makecell{30/30 \\ (113.5 $\pm$ 3.0)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (190.0)} % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b30-s5 &\wskip
  & \makecell{30/30 \\ (104.6 $\pm$ 3.5)} % ASNets
  & \makecell{30/30 \\ (110.4 $\pm$ 3.2)} % ASNets (PE)
  & \makecell{30/30 \\ (104.8 $\pm$ 3.2)} % ASNets (adm.)
  & \makecell{30/30 \\ (111.3 $\pm$ 2.4)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b35-s1 &\wskip
  & \makecell{30/30 \\ (131.6 $\pm$ 3.8)} % ASNets
  & \makecell{30/30 \\ (140.3 $\pm$ 4.5)} % ASNets (PE)
  & \makecell{30/30 \\ (132.3 $\pm$ 3.4)} % ASNets (adm.)
  & \makecell{30/30 \\ (132.8 $\pm$ 3.1)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b35-s2 &\wskip
  & \makecell{30/30 \\ (137.9 $\pm$ 3.8)} % ASNets
  & \makecell{30/30 \\ (147.8 $\pm$ 3.9)} % ASNets (PE)
  & \makecell{30/30 \\ (135.1 $\pm$ 4.1)} % ASNets (adm.)
  & \makecell{30/30 \\ (143.7 $\pm$ 3.2)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b35-s3 &\wskip
  & \makecell{30/30 \\ (120.2 $\pm$ 3.0)} % ASNets
  & \makecell{30/30 \\ (131.4 $\pm$ 4.2)} % ASNets (PE)
  & \makecell{30/30 \\ (115.7 $\pm$ 3.0)} % ASNets (adm.)
  & \makecell{30/30 \\ (125.1 $\pm$ 3.0)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b35-s4 &\wskip
  & \makecell{30/30 \\ (121.3 $\pm$ 2.8)} % ASNets
  & \makecell{30/30 \\ (131.5 $\pm$ 3.7)} % ASNets (PE)
  & \makecell{30/30 \\ (123.6 $\pm$ 3.4)} % ASNets (adm.)
  & \makecell{30/30 \\ (125.3 $\pm$ 3.2)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b35-s5 &\wskip
  & \makecell{30/30 \\ (133.6 $\pm$ 3.5)} % ASNets
  & \makecell{30/30 \\ (138.5 $\pm$ 3.6)} % ASNets (PE)
  & \makecell{30/30 \\ (134.4 $\pm$ 3.1)} % ASNets (adm.)
  & \makecell{30/30 \\ (130.3 $\pm$ 3.3)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b40-s1 &\wskip
  & \makecell{30/30 \\ (127.0 $\pm$ 3.5)} % ASNets
  & \makecell{30/30 \\ (140.9 $\pm$ 5.1)} % ASNets (PE)
  & \makecell{30/30 \\ (123.6 $\pm$ 2.9)} % ASNets (adm.)
  & \makecell{30/30 \\ (133.8 $\pm$ 3.0)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b40-s2 &\wskip
  & \makecell{30/30 \\ (147.1 $\pm$ 3.8)} % ASNets
  & \makecell{30/30 \\ (153.4 $\pm$ 3.1)} % ASNets (PE)
  & \makecell{30/30 \\ (144.4 $\pm$ 3.3)} % ASNets (adm.)
  & \makecell{30/30 \\ (149.9 $\pm$ 3.7)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b40-s3 &\wskip
  & \makecell{30/30 \\ (146.8 $\pm$ 4.1)} % ASNets
  & \makecell{30/30 \\ (160.0 $\pm$ 4.1)} % ASNets (PE)
  & \makecell{30/30 \\ (142.1 $\pm$ 3.8)} % ASNets (adm.)
  & \makecell{30/30 \\ (154.0 $\pm$ 4.2)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b40-s4 &\wskip
  & \makecell{30/30 \\ (152.2 $\pm$ 3.4)} % ASNets
  & \makecell{30/30 \\ (155.2 $\pm$ 4.1)} % ASNets (PE)
  & \makecell{30/30 \\ (144.8 $\pm$ 3.3)} % ASNets (adm.)
  & \makecell{30/30 \\ (151.8 $\pm$ 4.3)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
prob-bw-b40-s5 &\wskip
  & \makecell{30/30 \\ (144.9 $\pm$ 3.5)} % ASNets
  & \makecell{30/30 \\ (149.5 $\pm$ 3.9)} % ASNets (PE)
  & \makecell{30/30 \\ (143.1 $\pm$ 3.0)} % ASNets (adm.)
  & \makecell{30/30 \\ (145.8 $\pm$ 4.2)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\


==> results/prob-figures/ttw-0.tex <==
% ASNets & ASNets (PE) & ASNets (adm.) & ASNets (no h.) & LRTDP & LRTDP (adm.) & SSiPP & SSiPP (adm.) \\
triangle-tire-4 &\wskip
  & \makecell{30/30 \\ (23.4 $\pm$ 0.7)} % ASNets
  & \makecell{30/30 \\ (23.4 $\pm$ 0.7)} % ASNets (PE)
  & \makecell{30/30 \\ (23.4 $\pm$ 0.7)} % ASNets (adm.)
  & \makecell{30/30 \\ (23.4 $\pm$ 0.7)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (23.7 $\pm$ 0.7)} % LRTDP
  & \makecell{30/30 \\ (23.8 $\pm$ 0.6)} &\wskip % LRTDP (adm.)
  & \makecell{30/30 \\ (24.0 $\pm$ 0.7)} % SSiPP
  & \makecell{30/30 \\ (23.2 $\pm$ 0.7)} % SSiPP (adm.)
  \\
triangle-tire-5 &\wskip
  & \makecell{30/30 \\ (28.9 $\pm$ 0.8)} % ASNets
  & \makecell{30/30 \\ (28.9 $\pm$ 0.8)} % ASNets (PE)
  & \makecell{30/30 \\ (28.9 $\pm$ 0.8)} % ASNets (adm.)
  & \makecell{30/30 \\ (28.9 $\pm$ 0.8)} &\wskip % ASNets (no h.)
  & \makecell{30/30 \\ (30.7 $\pm$ 0.8)} % LRTDP
  & \makecell{19/30 \\ (29.1 $\pm$ 1.1)} &\wskip % LRTDP (adm.)
  & \makecell{29/30 \\ (30.8 $\pm$ 0.9)} % SSiPP
  & \makecell{30/30 \\ (30.2 $\pm$ 0.9)} % SSiPP (adm.)
  \\
triangle-tire-6 &\wskip
  & \makecell{30/30 \\ (34.9 $\pm$ 0.9)} % ASNets
  & \makecell{30/30 \\ (34.9 $\pm$ 0.9)} % ASNets (PE)
  & \makecell{30/30 \\ (34.9 $\pm$ 0.9)} % ASNets (adm.)
  & \makecell{30/30 \\ (34.9 $\pm$ 0.9)} &\wskip % ASNets (no h.)
  & \makecell{1/30 \\ (34.0)} % LRTDP
  & \makecell{1/30 \\ (34.0)} &\wskip % LRTDP (adm.)
  & \makecell{30/30 \\ (38.0 $\pm$ 0.8)} % SSiPP
  & \makecell{30/30 \\ (35.7 $\pm$ 0.8)} % SSiPP (adm.)
  \\
triangle-tire-7 &\wskip
  & \makecell{30/30 \\ (40.8 $\pm$ 0.9)} % ASNets
  & \makecell{30/30 \\ (40.8 $\pm$ 0.9)} % ASNets (PE)
  & \makecell{30/30 \\ (40.8 $\pm$ 0.9)} % ASNets (adm.)
  & \makecell{30/30 \\ (40.8 $\pm$ 0.9)} &\wskip % ASNets (no h.)
  & \makecell{1/30 \\ (42.0)} % LRTDP
  & \makecell{1/30 \\ (45.0)} &\wskip % LRTDP (adm.)
  & \makecell{27/30 \\ (45.5 $\pm$ 1.0)} % SSiPP
  & \makecell{16/30 \\ (41.7 $\pm$ 1.3)} % SSiPP (adm.)
  \\
triangle-tire-8 &\wskip
  & \makecell{30/30 \\ (46.8 $\pm$ 1.1)} % ASNets
  & \makecell{30/30 \\ (46.8 $\pm$ 1.1)} % ASNets (PE)
  & \makecell{30/30 \\ (46.8 $\pm$ 1.1)} % ASNets (adm.)
  & \makecell{30/30 \\ (46.8 $\pm$ 1.1)} &\wskip % ASNets (no h.)
  & \makecell{1/30 \\ (53.0)} % LRTDP
  & \makecell{1/30 \\ (50.0)} &\wskip % LRTDP (adm.)
  & \makecell{15/30 \\ (51.7 $\pm$ 1.2)} % SSiPP
  & \makecell{3/30 \\ (48.3 $\pm$ 7.6)} % SSiPP (adm.)
  \\
triangle-tire-9 &\wskip
  & \makecell{30/30 \\ (52.9 $\pm$ 1.3)} % ASNets
  & \makecell{30/30 \\ (52.9 $\pm$ 1.3)} % ASNets (PE)
  & \makecell{30/30 \\ (52.9 $\pm$ 1.3)} % ASNets (adm.)
  & \makecell{30/30 \\ (52.9 $\pm$ 1.3)} &\wskip % ASNets (no h.)
  & \makecell{1/30 \\ (59.0)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{3/30 \\ (60.7 $\pm$ 3.8)} % SSiPP
  & \makecell{1/30 \\ (55.0)} % SSiPP (adm.)
  \\
triangle-tire-10 &\wskip
  & \makecell{30/30 \\ (59.0 $\pm$ 1.1)} % ASNets
  & \makecell{30/30 \\ (59.0 $\pm$ 1.1)} % ASNets (PE)
  & \makecell{30/30 \\ (59.0 $\pm$ 1.1)} % ASNets (adm.)
  & \makecell{30/30 \\ (59.0 $\pm$ 1.1)} &\wskip % ASNets (no h.)
  & \makecell{1/30 \\ (69.0)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (67.0)} % SSiPP
  & - % SSiPP (adm.)
  \\
triangle-tire-11 &\wskip
  & \makecell{30/30 \\ (64.8 $\pm$ 1.1)} % ASNets
  & \makecell{30/30 \\ (64.8 $\pm$ 1.1)} % ASNets (PE)
  & \makecell{30/30 \\ (64.8 $\pm$ 1.1)} % ASNets (adm.)
  & \makecell{30/30 \\ (64.8 $\pm$ 1.1)} &\wskip % ASNets (no h.)
  & \makecell{1/30 \\ (75.0)} % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (77.0)} % SSiPP
  & - % SSiPP (adm.)
  \\
triangle-tire-12 &\wskip
  & \makecell{30/30 \\ (71.1 $\pm$ 1.2)} % ASNets
  & \makecell{30/30 \\ (71.1 $\pm$ 1.2)} % ASNets (PE)
  & \makecell{30/30 \\ (71.1 $\pm$ 1.2)} % ASNets (adm.)
  & \makecell{30/30 \\ (71.1 $\pm$ 1.2)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & \makecell{1/30 \\ (79.0)} % SSiPP
  & - % SSiPP (adm.)
  \\
triangle-tire-13 &\wskip
  & \makecell{30/30 \\ (76.9 $\pm$ 1.2)} % ASNets
  & \makecell{30/30 \\ (76.9 $\pm$ 1.2)} % ASNets (PE)
  & \makecell{30/30 \\ (76.9 $\pm$ 1.2)} % ASNets (adm.)
  & \makecell{30/30 \\ (76.9 $\pm$ 1.2)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
triangle-tire-14 &\wskip
  & \makecell{30/30 \\ (82.8 $\pm$ 1.3)} % ASNets
  & \makecell{30/30 \\ (82.8 $\pm$ 1.3)} % ASNets (PE)
  & \makecell{30/30 \\ (82.8 $\pm$ 1.3)} % ASNets (adm.)
  & \makecell{30/30 \\ (82.8 $\pm$ 1.3)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
triangle-tire-15 &\wskip
  & \makecell{30/30 \\ (88.7 $\pm$ 1.4)} % ASNets
  & \makecell{30/30 \\ (88.7 $\pm$ 1.4)} % ASNets (PE)
  & \makecell{30/30 \\ (88.7 $\pm$ 1.4)} % ASNets (adm.)
  & \makecell{30/30 \\ (88.7 $\pm$ 1.4)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
triangle-tire-16 &\wskip
  & \makecell{30/30 \\ (94.8 $\pm$ 1.3)} % ASNets
  & \makecell{30/30 \\ (94.8 $\pm$ 1.3)} % ASNets (PE)
  & \makecell{30/30 \\ (94.8 $\pm$ 1.3)} % ASNets (adm.)
  & \makecell{30/30 \\ (94.8 $\pm$ 1.3)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
triangle-tire-17 &\wskip
  & \makecell{30/30 \\ (100.8 $\pm$ 1.2)} % ASNets
  & \makecell{30/30 \\ (100.8 $\pm$ 1.2)} % ASNets (PE)
  & \makecell{30/30 \\ (100.8 $\pm$ 1.2)} % ASNets (adm.)
  & \makecell{30/30 \\ (100.8 $\pm$ 1.2)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
triangle-tire-18 &\wskip
  & \makecell{30/30 \\ (106.5 $\pm$ 1.4)} % ASNets
  & \makecell{30/30 \\ (106.5 $\pm$ 1.4)} % ASNets (PE)
  & \makecell{30/30 \\ (106.5 $\pm$ 1.4)} % ASNets (adm.)
  & \makecell{30/30 \\ (106.5 $\pm$ 1.4)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
triangle-tire-19 &\wskip
  & \makecell{30/30 \\ (112.5 $\pm$ 1.6)} % ASNets
  & \makecell{30/30 \\ (112.5 $\pm$ 1.6)} % ASNets (PE)
  & \makecell{30/30 \\ (112.5 $\pm$ 1.6)} % ASNets (adm.)
  & \makecell{30/30 \\ (112.5 $\pm$ 1.6)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\
triangle-tire-20 &\wskip
  & \makecell{30/30 \\ (118.4 $\pm$ 1.5)} % ASNets
  & \makecell{30/30 \\ (118.4 $\pm$ 1.5)} % ASNets (PE)
  & \makecell{30/30 \\ (118.4 $\pm$ 1.5)} % ASNets (adm.)
  & \makecell{30/30 \\ (118.4 $\pm$ 1.5)} &\wskip % ASNets (no h.)
  & - % LRTDP
  & - &\wskip % LRTDP (adm.)
  & - % SSiPP
  & - % SSiPP (adm.)
  \\


==> tables/parking.tex <==
%\begin{landscape}
  \begin{table}
    \begin{center}
      \begin{scriptsize}
        \begin{tabular}{@{}lccccccccccccc@{}}
        \toprule
        \multirow{2}{*}{Problem}\wskip&
          & \multicolumn{3}{c}{ASNet} \wskip&
          & \multicolumn{2}{c}{A*}\wskip&
          & \multicolumn{1}{c}{GBF}\wskip&
          & \multicolumn{2}{c}{LAMA}
          \\
          \cmidrule{3-5} \cmidrule{7-8} \cmidrule{10-10} \cmidrule{12-13}
          &\wskip & - & PE & No LM
          &\wskip & LM-cut & h-add
          &\wskip & LM-cut
          &\wskip & -2011 & -first
          % &\wskip & h-add & LM-cut &\wskip & h-add & LM-cut
          \\
          \midrule
% ASNets & ASNets (PE) & ASNets (no LM) & A* (adm.) & A* (inadm.) & GBF (adm.) & LAMA-2011 & LAMA-first \\
parking-c10-10 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 37 &\wskip % A* (inadm.)
  & 57 &\wskip % GBF (adm.)
  & 30 % LAMA-2011
  & 55 % LAMA-first
  \\
parking-c10-08 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 39 &\wskip % A* (inadm.)
  & 48 &\wskip % GBF (adm.)
  & 28 % LAMA-2011
  & 53 % LAMA-first
  \\
parking-c10-05 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 66 &\wskip % GBF (adm.)
  & 27 % LAMA-2011
  & 49 % LAMA-first
  \\
parking-c10-07 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 59 &\wskip % GBF (adm.)
  & 29 % LAMA-2011
  & 59 % LAMA-first
  \\
parking-c10-09 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 56 &\wskip % GBF (adm.)
  & 29 % LAMA-2011
  & 53 % LAMA-first
  \\
parking-c12-08 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 80 &\wskip % GBF (adm.)
  & 42 % LAMA-2011
  & 72 % LAMA-first
  \\
parking-c12-10 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 80 &\wskip % GBF (adm.)
  & 38 % LAMA-2011
  & 75 % LAMA-first
  \\
parking-c12-07 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 47 &\wskip % A* (inadm.)
  & 78 &\wskip % GBF (adm.)
  & 67 % LAMA-2011
  & 57 % LAMA-first
  \\
parking-c12-09 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 42 &\wskip % A* (inadm.)
  & 73 &\wskip % GBF (adm.)
  & 32 % LAMA-2011
  & 48 % LAMA-first
  \\
parking-c12-06 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 73 &\wskip % GBF (adm.)
  & 37 % LAMA-2011
  & 76 % LAMA-first
  \\
parking-c13-07 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 90 &\wskip % GBF (adm.)
  & 39 % LAMA-2011
  & 73 % LAMA-first
  \\
parking-c13-06 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 72 &\wskip % GBF (adm.)
  & 66 % LAMA-2011
  & 68 % LAMA-first
  \\
parking-c13-08 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 70 &\wskip % GBF (adm.)
  & 62 % LAMA-2011
  & 81 % LAMA-first
  \\
parking-c13-10 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 69 &\wskip % GBF (adm.)
  & 37 % LAMA-2011
  & 77 % LAMA-first
  \\
parking-c13-09 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 44 &\wskip % A* (inadm.)
  & 61 &\wskip % GBF (adm.)
  & 57 % LAMA-2011
  & 58 % LAMA-first
  \\
parking-c15-04 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 68 &\wskip % GBF (adm.)
  & 78 % LAMA-2011
  & 74 % LAMA-first
  \\
parking-c15-03 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 51 &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 58 % LAMA-2011
  & 93 % LAMA-first
  \\
parking-c15-09 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 70 % LAMA-2011
  & 59 % LAMA-first
  \\
parking-c15-01 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 79 % LAMA-2011
  & 83 % LAMA-first
  \\
parking-c15-10 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 53 % LAMA-2011
  & 67 % LAMA-first
  \\
parking-c15-07 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 84 % LAMA-2011
  & 84 % LAMA-first
  \\
parking-c15-02 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 52 % LAMA-2011
  & 98 % LAMA-first
  \\
parking-c15-05 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 67 % LAMA-2011
  & 88 % LAMA-first
  \\
parking-c15-06 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 51 % LAMA-2011
  & 95 % LAMA-first
  \\
parking-c15-08 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 65 % LAMA-2011
  & 84 % LAMA-first
  \\
parking-c20-05 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 63 % LAMA-2011
  & 91 % LAMA-first
  \\
parking-c20-04 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 97 % LAMA-2011
  & 128 % LAMA-first
  \\
parking-c20-02 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 90 % LAMA-2011
  & 103 % LAMA-first
  \\
parking-c20-01 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 63 % LAMA-2011
  & 122 % LAMA-first
  \\
parking-c20-03 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & - &\wskip % GBF (adm.)
  & 62 % LAMA-2011
  & 115 % LAMA-first
  \\
\bottomrule
        \end{tabular}
      \end{scriptsize}
    \end{center}
    \caption{
    more captions for unfinished parking results
  }
  \label{tab:det-res-parking}
  \end{table}
  %\end{landscape}

==> tables/sokoban.tex <==
%\begin{landscape}
  \begin{table}
    \begin{center}
      \begin{scriptsize}
        \begin{tabular}{@{}lccccccccccccc@{}}
        \toprule
        \multirow{2}{*}{Problem}\wskip&
          & \multicolumn{3}{c}{ASNet} \wskip&
          & \multicolumn{2}{c}{A*}\wskip&
          & \multicolumn{1}{c}{GBF}\wskip&
          & \multicolumn{2}{c}{LAMA}
          \\
          \cmidrule{3-5} \cmidrule{7-8} \cmidrule{10-10} \cmidrule{12-13}
          &\wskip & - & PE & No LM
          &\wskip & LM-cut & h-add
          &\wskip & LM-cut
          &\wskip & -2011 & -first
          % &\wskip & h-add & LM-cut &\wskip & h-add & LM-cut
          \\
          \midrule
% NB: all the problem names originally had "-w04-" before the final two digits.  I don't know the significance of that designator. Also, they all had -n09 in their names after "sokoban" originally.
% ASNets & ASNets (PE) & ASNets (no LM) & A* (adm.) & A* (inadm.) & GBF (adm.) & LAMA-2011 & LAMA-first \\
sokoban-b03-01 &\wskip
  & - % ASNets
  & 150 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 51 % A* (adm.)
  & 51 &\wskip % A* (inadm.)
  & 67 &\wskip % GBF (adm.)
  & 51 % LAMA-2011
  & 99 % LAMA-first
  \\
sokoban-b03-02 &\wskip
  & - % ASNets
  & 174 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 68 % A* (adm.)
  & 68 &\wskip % A* (inadm.)
  & 160 &\wskip % GBF (adm.)
  & 68 % LAMA-2011
  & 112 % LAMA-first
  \\
sokoban-b03-03 &\wskip
  & - % ASNets
  & 87.4 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 57 % A* (adm.)
  & 57 &\wskip % A* (inadm.)
  & 89 &\wskip % GBF (adm.)
  & 57 % LAMA-2011
  & 79 % LAMA-first
  \\
sokoban-b03-04 &\wskip
  & - % ASNets
  & 131 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 59 % A* (adm.)
  & 59 &\wskip % A* (inadm.)
  & 85 &\wskip % GBF (adm.)
  & 59 % LAMA-2011
  & 71 % LAMA-first
  \\
sokoban-b03-05 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 62 % A* (adm.)
  & 64 &\wskip % A* (inadm.)
  & 94 &\wskip % GBF (adm.)
  & 62 % LAMA-2011
  & 150 % LAMA-first
  \\
sokoban-b03-06 &\wskip
  & - % ASNets
  & 118.5 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 56 % A* (adm.)
  & 56 &\wskip % A* (inadm.)
  & 92 &\wskip % GBF (adm.)
  & 56 % LAMA-2011
  & 104 % LAMA-first
  \\
sokoban-b03-07 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 68 % A* (adm.)
  & 68 &\wskip % A* (inadm.)
  & 160 &\wskip % GBF (adm.)
  & 68 % LAMA-2011
  & 112 % LAMA-first
  \\
sokoban-b03-08 &\wskip
  & - % ASNets
  & 89.8 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 59 % A* (adm.)
  & 59 &\wskip % A* (inadm.)
  & 85 &\wskip % GBF (adm.)
  & 59 % LAMA-2011
  & 69 % LAMA-first
  \\
sokoban-b03-09 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 59 % A* (adm.)
  & 59 &\wskip % A* (inadm.)
  & 99 &\wskip % GBF (adm.)
  & 59 % LAMA-2011
  & 81 % LAMA-first
  \\
sokoban-b03-10 &\wskip
  & - % ASNets
  & 129 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & 55 % A* (adm.)
  & 55 &\wskip % A* (inadm.)
  & 99 &\wskip % GBF (adm.)
  & 55 % LAMA-2011
  & 71 % LAMA-first
  \\
sokoban-b04-01 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 74 &\wskip % A* (inadm.)
  & 144 &\wskip % GBF (adm.)
  & 74 % LAMA-2011
  & 116 % LAMA-first
  \\
sokoban-b04-02 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 187 &\wskip % GBF (adm.)
  & 83 % LAMA-2011
  & 179 % LAMA-first
  \\
sokoban-b04-03 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 134 &\wskip % GBF (adm.)
  & 76 % LAMA-2011
  & 108 % LAMA-first
  \\
sokoban-b04-04 &\wskip
  & - % ASNets
  & 178 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 138 &\wskip % GBF (adm.)
  & 78 % LAMA-2011
  & 200 % LAMA-first
  \\
sokoban-b04-05 &\wskip
  & - % ASNets
  & 122 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 277 &\wskip % GBF (adm.)
  & 83 % LAMA-2011
  & 163 % LAMA-first
  \\
sokoban-b04-06 &\wskip
  & - % ASNets
  & 180.6 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 149 &\wskip % GBF (adm.)
  & 75 % LAMA-2011
  & 111 % LAMA-first
  \\
sokoban-b04-07 &\wskip
  & - % ASNets
  & 179 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 227 &\wskip % GBF (adm.)
  & 93 % LAMA-2011
  & 141 % LAMA-first
  \\
sokoban-b04-08 &\wskip
  & - % ASNets
  & 215 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 153 &\wskip % GBF (adm.)
  & 79 % LAMA-2011
  & 95 % LAMA-first
  \\
sokoban-b04-09 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 255 &\wskip % GBF (adm.)
  & 81 % LAMA-2011
  & 179 % LAMA-first
  \\
sokoban-b04-10 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 159 &\wskip % GBF (adm.)
  & 77 % LAMA-2011
  & 141 % LAMA-first
  \\
sokoban-b04-11 &\wskip
  & - % ASNets
  & 77 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 139 &\wskip % GBF (adm.)
  & 69 % LAMA-2011
  & 77 % LAMA-first
  \\
sokoban-b04-12 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 155 &\wskip % GBF (adm.)
  & 87 % LAMA-2011
  & 129 % LAMA-first
  \\
sokoban-b04-13 &\wskip
  & - % ASNets
  & 138 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 292 &\wskip % GBF (adm.)
  & 82 % LAMA-2011
  & 128 % LAMA-first
  \\
sokoban-b04-14 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 156 &\wskip % GBF (adm.)
  & 86 % LAMA-2011
  & 132 % LAMA-first
  \\
sokoban-b04-15 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 166 &\wskip % GBF (adm.)
  & 84 % LAMA-2011
  & 174 % LAMA-first
  \\
sokoban-b04-16 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 134 &\wskip % GBF (adm.)
  & 84 % LAMA-2011
  & 138 % LAMA-first
  \\
sokoban-b04-17 &\wskip
  & - % ASNets
  & 185 % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 149 &\wskip % GBF (adm.)
  & 79 % LAMA-2011
  & 245 % LAMA-first
  \\
sokoban-b04-18 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 67 &\wskip % A* (inadm.)
  & 127 &\wskip % GBF (adm.)
  & 67 % LAMA-2011
  & 83 % LAMA-first
  \\
sokoban-b04-19 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & 73 &\wskip % A* (inadm.)
  & 155 &\wskip % GBF (adm.)
  & 73 % LAMA-2011
  & 89 % LAMA-first
  \\
sokoban-b04-20 &\wskip
  & - % ASNets
  & - % ASNets (PE)
  & - &\wskip % ASNets (no LM)
  & - % A* (adm.)
  & - &\wskip % A* (inadm.)
  & 127 &\wskip % GBF (adm.)
  & 73 % LAMA-2011
  & 93 % LAMA-first
  \\
\bottomrule
        \end{tabular}
      \end{scriptsize}
    \end{center}
    \caption{
    more captions for unfinished sokoban results
  }
  \label{tab:det-res-sokoban}
  \end{table}
  %\end{landscape}
